Auto-FuzzyJoin: Auto-Program Fuzzy Similarity Joins Without Labeled Examples

Fuzzy similarity join is an important database operator widely used in practice. So far the research community has focused exclusively on optimizing fuzzy join \textit{scalability}. However, practitioners today also struggle to optimize fuzzy-join \textit{quality}, because they face a daunting space of parameters (e.g., distance-functions, distance-thresholds, tokenization-options, etc.), and often have to resort to a manual trial-and-error approach to program these parameters in order to optimize fuzzy-join quality. This key challenge of automatically generating high-quality fuzzy-join programs has received surprisingly little attention thus far. In this work, we study the problem of "auto-program" fuzzy-joins. Leveraging a geometric interpretation of distance-functions, we develop an unsupervised \textsc{Auto-FuzzyJoin} framework that can infer suitable fuzzy-join programs on given input tables, without requiring explicit human input such as labeled training data. Using \textsc{Auto-FuzzyJoin}, users only need to provide two input tables $L$ and $R$, and a desired precision target $\tau$ (say 0.9). \textsc{Auto-FuzzyJoin} leverages the fact that one of the input is a reference table to automatically program fuzzy-joins that meet the precision target $\tau$ in expectation, while maximizing fuzzy-join recall (defined as the number of correctly joined records). Experiments on both existing benchmarks and a new benchmark with 50 fuzzy-join tasks created from Wikipedia data suggest that the proposed \textsc{Auto-FuzzyJoin} significantly outperforms existing unsupervised approaches, and is surprisingly competitive even against supervised approaches (e.g., Magellan and DeepMatcher) when 50\% of ground-truth labels are used as training data.

==> Algorithm.tex <==
\section{Algorithms}

The whole procedure of our greedy algorithm includes the following parts: preprocessing, blocking, distance calculating, threshold pruning and configuration selecting. The the rest part of section, we will introduce each steps' detailed implementation give our pseudo code.


\subsection{ Preprocessing} 

Our preprocessing procedure contains four steps, each step takes a string as input and outputs a string after preprocessing. Each step of preprocessing are listed in table 1. 

\begin{table}
\centering
  \caption{Preprocessing Method Space}
  \begin{tabular}{|c|l|} \hline
    Dimensions&Methods\\ \hline
    1&None, lower case\\ \hline
    2&None, stop word\\ \hline
    3&None, punctuation\\ \hline
    4&None, stemming, lemmatization\\ \hline
    \hline\end{tabular}
\end{table}

According to methods described above, our preprocessing step works like this:

\begin{algorithm}
\caption{Preprocessing algorithm}\label{euclid}
\begin{algorithmic}[1]
\Procedure{DoPreprocessing}{}
\State $\textit{left} \gets \text{left input table}$
\State $\textit{right} \gets \text{right input table}$

\ForAll $\textit{lvalue} \in \mathcal \textit{left} $
\ForAll $\textit{method} \in \mathcal \textit{method\_space}$
\State $\textit{lvalue} \gets apply(\textit{method}, \textit{lvalue})$
\EndFor
\EndFor

\ForAll $\textit{rvalue} \in \mathcal \textit{right} $
\ForAll$\textit{method} \in \mathcal \textit{method\_space}$
\State $\textit{rvalue} \gets apply(\textit{method}, \textit{rvalue})$
\EndFor
\EndFor

\EndProcedure
\end{algorithmic}
\end{algorithm}















\bigskip

\subsection{Blocking} 
Our algorithm uses blocking to decrease the number of potential candidate pairs. Without blocking, the number of potential candidate pairs are $n_L$ * $n_R$, the cross products of left table and right table. However,  we could use several simple rules to cut down the number of candidate pairs:


\begin{itemize}
    \item \at{1.} For our potential joining pairs, we expect they have at least one shared token or word. The tokenization methods include word tokenization, 3-gram and 4-gram. These methods could probably cover all potential conditions. And if two candidate pairs don't share one token or word, it's impossible to join them using fuzzy join.
    \item \at{1.} The shared token or word should have a low frequency among the whole table. This rule is trying to apply a more strict constraint to decrease the number of candidates. Here we use this rule to control the number of candidates after blocking.
\end{itemize}

Based on rules described above, we could control our blocking table's size by setting the maximum threshold for the shared tokens. The pseudo code of blocking method works like this:

\begin{algorithm}
\caption{Blocking algorithm}\label{euclid}
\begin{algorithmic}[1]
\Procedure{DoBlocking}{}
\State $\textit{left} \gets \text{left input table}$
\State $\textit{right} \gets \text{right input table}$
\State $\textit{token\_lid\_map} \gets \text{map}$
\State $\textit{joined\_table} \gets \text{set}$
\ForAll $\textit{lid, lvalue} \in \mathcal \textit{left} $
\State $\textit{ltokens} \gets \text{word\_token(\textit{lvalue}) \textit{UNION} Ngram\_token(\textit{lvalue})} $
\ForAll $\textit{token} \in \mathcal \textit{ltokens}$
\State $\text{\textit{token\_lid\_map[token]} = \textit{token\_lid\_map[token]} UNION \textit{lid}}$
\EndFor
\EndFor


\State $\textit{token\_max\_freq} \gets \sqrt{\textit{left.length}}$
\ForAll $\textit{rid, rvalue} \in \mathcal \textit{right} $
\State $\textit{rtokens} \gets \text{word\_token(\textit{rvalue}) \textit{UNION} Ngram\_token(\textit{rvalue})} $
\ForAll $\textit{token} \in \mathcal \textit{rtokens}$
\If{\textit{token} \textbf{in} \textit{token\_lid\_map}}
\ForAll $\textit{lid} \in \mathcal \textit{token\_lid\_map[token]}$
\State $\textit{joined\_table}.add(<\textit{lid}, \textit{rid}>)$
\EndFor
\EndIf
\EndFor
\EndFor

\EndProcedure
\end{algorithmic}
\end{algorithm}















\bigskip

\subsection{Distance Calculating}
After previous work done, we now have a joined table of all possible candidate pairs and we are going to calculate the distance between each records. Based on the distance, we could find the appropriate joining threshold from left table self joins and apply the threshold to the left right table join. State-of-art methods to perform calculation could be divided into 2 categories, string based method and set based method. In this section, we will talk about these to categories individually and combine them together to our full method space.

\subsubsection{String Distance}

We define string distance method as the method whose input is 2 strings and outputs the distance of the two strings.  

% todo we need a abstract of state-of-art introduction here

Among the previous state-of-art methods, we pick 2 of them in our method space. The methods we choose are editdistance and jaro-winker distance. The algorithm to calculate string distance is quite straight :

\begin{algorithm}
\caption{String distance calculating}\label{euclid}
\begin{algorithmic}[1]
\Procedure{CalculateStringDistance}{}
\State $\textit{joined\_table} \gets \text{joined table output by blocking}$
\ForAll $\textit{lvalue, rvalue} \in \mathcal \textit{joined\_table}$
\State $\textit{distance} \gets string\_distance(\textit{lvalue, rvalue})$
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

\subsubsection{Set Distance}

Set distance methods are quite different from string distance methods. In fact, set distance methods are combinations of methods to calculate the distance between 2 strings. Here the whole process could be divided into 4 steps: tokenizing, token weighting, number weighting \& similarity calculating.  In each step, we need to test a combination of 4 methods to calculate the distance among joined tables.

\begin{table}
\centering
  \caption{Set Distance Method Space}
  \begin{tabular}{|c|c|l|} \hline
    Steps&Name&Methods\\ \hline
    1&Tokenization&word, 2-gram, 3-gram, 4-gram\\ \hline
    2&Token\_Weight&None, IDF, OPT\_IDF\\ \hline
    3&Number\_Token\_Weight&0.5, 1, 2, 4\\ \hline
    4&Similarity&intersection, jaccard, jaccard\_containment, cosine, dice, max\_include\\ \hline
    \hline\end{tabular}
\end{table}

% todo: where & how to introduce our self defined weight method
\begin{algorithm}
\caption{Set distance calculating}\label{euclid}
\begin{algorithmic}[1]
\Procedure{CalculateSetDistance}{}
\State $\textit{joined\_table} \gets \text{joined table output by blocking}$
\ForAll $\textit{tokenize, token\_weight, num\_weight, similarity\_method} \in \mathcal \textit{all\_possible\_methods}$
% \ForAll{$\textit{token\_weight\_method} \in \mathcal \textit{all\_possible\_token\_weight\_method}$}
% \ForAll{$\textit{num\_weight\_method} \in \mathcal \textit{all\_possible\_num\_weight\_method}$}
% \ForAll{$\textit{similarity\_method} \in \mathcal \textit{all\_possible\_similarity\_method}$}

\State $\textit{weight\_map} \gets apply(\textit{joined\_table, token\_weight\_method, num\_weight\_method})$

\ForAll $\textit{lvalue, rvalue} \in \mathcal \textit{joined\_table}$
\State $\textit{ltokens} \gets tokenize\_method(\textit{lvalue})$
\State $\textit{rtokens} \gets tokenize\_method(\textit{rvalue})$

\State $\textit{distance} \gets similarity\_method(\textit{ltokens, rtokens, weight\_map})$


% \EndFor
% \EndFor
% \EndFor
\EndFor
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}


\subsection{Profit Based Selection}

After previous calculation done, we could have a set of configurations and their results applying to joined table. So our algorithm is going to select the best configuration from the previous search space. 
% todo: add our intuitive description, using left to describe right







==> AutoFJJoinRules.tex <==

\section{AutoFJ Setup}
In this section, we first introduced how to produce a fuzzy join based on single distance measurement. We then design a set of rules to produce a fuzzy join using multiple distance measurements. 




\subsection{Solution Space}

A solution is a list of $\big( \langle f_1, \theta_1\rangle, \langle f_2, \theta_2\rangle, \ldots, \langle f_k, \theta_k\rangle  \big)$, where $f_j, j \in [1,k]$ is one of the distance functions introduced in the previous subsection. 


Resolving conflicts. two cases: 

\subsection{Simple Join Rules}
Each configuration $C$ and weight-column vector $w$ (for multi-column joins) produces a real number indicating the distance for a pair of records. To determine whether they should be joined or not, a cut-off threshold value $\theta$ needs to be inferred to distinguish joining pairs from non-joining pairs. With the distance and threshold, we formally define the joining rule as follows:

\begin{definition}
Let $l$ be one record in table $L$ and $r$ be one record in table $R$. The distance between $l$ and $r$ is $d$ and the cut-off theshold is $\theta$. Then $l$ and $r$ can be joined only if the following two conditions are satisfied:

\begin{itemize}
    \item $d \leq \theta$ 
    \item There does not exist another record $l' \in L, l' \neq l$, such that $distance(l', r) < d$.
\end{itemize}

We denote the above rules as a function $\mathcal{J}$: ($d$, $\theta$) $\rightarrow$ bool, indicating whether $l$ and $r$ can be joined or not.
\end{definition}

The second condition results from the many-to-one join assumption. Since at most one record from $L$ can be joined with each record from $R$, we only select the record from $L$ with the smallest distance to be joined. If there exist ties, no records from $L$ will be joined. 

\subsection{AutoFJ Join Rules}


\textcolor{red}{need to explain why we use disjunction here??}
\bigskip
By combining definition 2 to 4, we proposed a \textit{fuzzy join package} formally defined as follows:
\begin{definition}
A \em{fuzzy join package} ${\cal Z}$ includes a column-weight vector $w$ and a list of 2-tuples [$\langle C_1, \theta_1 \rangle$, $\langle C_2, \theta_2 \rangle$ ...], where $C_i \in {\cal C}$ is a configuration and $\theta_i \in \mathbb{R}$ is a cut-off threshold. ${\cal Z}$ joins a record $r \in R$  with a record $l \in L$ only if the following two conditions are satisfied: 
\begin{itemize}
    \item There exists a 2-tuple $\langle C_i, \theta_i \rangle$ in ${\cal Z}$, such that $\mathcal{J}(D(w, C_i, l, r), \theta_i) = TRUE$
    \item There does not exist another record $l' \in L, l' \neq l$ and a 2-tuple $\langle C_j, \theta_j \rangle$ $j < i$, in ${\cal Z}$, such that $\mathcal{J}(D(w, C_j, l', r), \theta_j) = TRUE$
\end{itemize}
\end{definition}

The second condition is used to solve the conflicts where two configurations and thresholds select different $l$ to be joined. In this case, the first one in the package wins.


==> ComputePrecision.tex <==
\section{Estimate Precision}



==> RevisionCoverLetter.tex <==
% \documentclass[sigconf]{acmart}
% \settopmatter{printacmref=false} % Removes citation information below abstract
% \renewcommand\footnotetextcopyrightpermission[1]{} % removes footnote with conference information in first column
% %%
% %% \BibTeX command to typeset BibTeX logo in the docs
% \AtBeginDocument{%
%   \providecommand\BibTeX{{%
%     \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}
    
% \usepackage{comment}
% \usepackage{xspace}
% \usepackage{url}
% \usepackage{graphicx}
% \usepackage{balance}  % for  \balance command ON LAST PAGE  (only there!)
% \usepackage{xcolor}
% \usepackage{amsmath}
% %\usepackage{algpseudocode}
% \usepackage{enumitem}
% \usepackage[noend]{algorithmic}
% \usepackage{algorithm}
% \usepackage{subfigure}
% %\usepackage{subcaption}
% %\usepackage{caption,subcaption}
% \usepackage{cleveref}
% \usepackage{url}
% \usepackage{multirow}
% \usepackage{amsmath}
% % \usepackage{subcaption}

% \newcommand\xu[1]{\textcolor{purple}{(Xu) #1} }



% \newcommand{\stitle}[1]{\vspace{1ex}\noindent{\bf #1}}
% \makeatletter
% \DeclareRobustCommand*\cal{\@fontswitch\relax\mathcal}
% \makeatother

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

% \sloppy
% \begin{document}
% \title{Auto-FuzzyJoin:\\ Auto-Tune Fuzzy Joins Without Labeled Examples}
% \author{(Revision Letter)}

% \maketitle

% \bigskip
\begin{center}
    {\LARGE Revision for SIGMOD'21 Paper 140: \\Auto-FuzzyJoin:Auto-Tune Fuzzy Joins Without Labeled Examples}

\end{center}

We would like to thank all reviewers for their insightful feedback and the opportunity to revise. In our revised manuscript, we have highlighted \rev{our revised sections in blue}. As suggested by the meta-reviewer, our experiments are made reproducible using the code shared via the link we submitted with the paper. 
%We conducted additional experiments and improved writings of the paper to address all comments from the reviewers. In this letter, we describe the major changes that we have made in our revision:

% \begin{enumerate}
% \item Reviewers' comments are in \textbf{black, bold font};
% \item General discussions are in black font;
% \item Concrete changes in the revision are in \textcolor{blue}{blue font}.
% \end{enumerate}

\bigskip
{\huge \stitle{Response to Comments by Reviewer 1}}

\bigskip
\begin{tcolorbox}
\textbf{O1: It is unclear to me how configurations are selected by the algorithm automatically. For example, in Sec. 3.2 there are two iterations of the algorithm, in each a different set of similarity metrics is chosen to determine which records can be joined. Is there a catalog of configurations that the greedy algorithm chooses from? Are these configurations specified by the user or the system? What if there are multiple configurations that generate the same precision/recall values, how do you choose which is the best?}
\end{tcolorbox}


\stitle{Response.} 

\begin{itemize}
    \item There is indeed a catalog of configurations derived from the Fuzzy-Join literature (e.g.,~\cite{chaudhuri_icde06, Sarawagi_sigmod04, doan2012principles}). Out of the box, the system has a total of 140 discrete join configurations (each also have continuous score-thresholds that are dynamically-tuned),  which is shown in  Table \ref{table:paramter_options} (copied below for reference). Details of these options in the configuration space are discussed in detail in Figure~\ref{fig:taxonomy_parameter} and Section \ref{sec:alg_compared} of our paper.
    
\vspace{-2mm}
\begin{table}[!h]
\centering
\scalebox{0.65}{
\begin{tabular}{|c|c|c|}
\hline
\multicolumn{2}{|c|}{\textbf{Parameters}} & \textbf{Values} \\ \hline
\multicolumn{2}{|c|}{Preprocessing} & L, L+S, L+RP, L+S+RP \\ \hline
\multicolumn{2}{|c|}{Tokenization} & 3G, SP \\ \hline
\multicolumn{2}{|c|}{Token Weights} & EW, IDFW \\ \hline
\multirow{6}{*}{Distance Function} & Character-based & JW, ED \\ \cline{2-3} 
 & \multirow{4}{*}{Set-based} & JD, CD, MD, DD, ID \\ \cline{3-3} 
 &  & *Contain-Jaccard \\ \cline{3-3} 
 &  & *Contain-Cosine \\ \cline{3-3} 
 &  & *Contain-Dice Distance \\ \cline{2-3} 
 & Embedding & GED \\ \hline
\end{tabular}
}
\caption*{Taken from Table \ref{table:paramter_options} of our paper: Configuration space of all discrete options (a cross-product produces 140 configurations). Details of each of these options are described in Figure~\ref{fig:taxonomy_parameter} and Section \ref{sec:alg_compared}.}
% \label{table:paramter_options}
\vspace{-6mm}
\end{table}


    \item In addition to the system-provided configurations, users can also extend this configuration space, by either adding customized configurations  tailored to their domains (e.g., new distance functions such as GED shown in the table above which is a Word2Vec-like distance), or removing distance functions that are known to be sub-optimal for their domains. To demonstrate this point empirically,
    we added an experiment in \rev{Section \ref{sec:single_column_evaluation_results} (under "Varying Configuration Spaces")} of our revised paper, which performs auto-fuzzy-joins using a varying number of configurations (varying from 24 to 140 configurations). We showed that a larger number of configurations leads to better join quality, at the cost of a slightly increased running time. This demonstrates that our proposed algorithm can indeed make use of a larger space of configurations and discover better fuzzy-joins when more configurations are made available to the algorithm.
    
    %-- for example in experiments we added Word2Vec embedding distance, which is not used in typical fuzzy-joins.
    
    \item Configurations with the same precision/recall -- In choosing  between candidate configurations (Line 9 of Algorithm \ref{alg:autofj_single_column}), if we encounter multiple configurations with the same estimated precision/recall values, we break ties by picking randomly, which is fairly standard in similar optimization algorithms. We should highlight that on large datasets, ties rarely happen, and when they do happen the specific choice of which configuration to use typically does not matter as these configurations often lead to the same join results (and thus identical precision/recall scores in the end). We have clarified these details \rev{in the description of Algorithm \ref{alg:autofj_single_column} in Section~\ref{sec:auto_fj_algorithm_single_column}.} We also validate this empirically by running our algorithm 5 times on 50 single-column datasets with different random seeds for breaking ties. The average precision ranges from 0.885 to 0.888 and the average recall ranges from 0.624 to 0.626, which shows that the randomly tie-breaking indeed has minimal impact on results.
    
    % \color{red}{Can we try run our algorithms 5 times and report variances, to show that random tie-breaking indeed does not matter?}
\end{itemize}


\bigskip
\begin{tcolorbox}
\textbf{O2: According to Sec 3.1, precision and recall vary depending on the configuration and (presumably) the dataset. Later on the authors mention that estimated precision/recall computation is done as a pre-processing step. How much time does this step take? How much time does it take to compute the precision/recall values during the algorithm execution of AutoFJ? I'm assuming that the use case for this work is interactive fuzzy joins, similar to Excel. Can your greedy algorithm deliver near real-time performance?}
\end{tcolorbox}

\stitle{Response.}
\begin{itemize}
    \item This is a clarification we should make to strengthen the paper. Because precision estimation is required in all iterations, we indeed optimize this by pre-computing these values upfront, and then performing lookups in subsequent iterations. In the revision, we provide a complexity analysis of this pre-computation \rev{at the end of Section \ref{sec:auto_fj_algorithm_single_column}},
    and we report that the running time of this pre-computation to be less than 10\% of the overall time of Algorithm \ref{alg:autofj_single_column} (shown in \rev{Figure \ref{fig:vary_space_efficiency}}). In contrast, if we do not use this optimization and compute these scores repeatedly in each iteration, our overall latency of Algorithm \ref{alg:autofj_single_column} is around 6x slower (with this component taking ~85\% time). We have now added more discussions of this optimization and highlighted its importance in \rev{Section \ref{sec:single_column_evaluation_results}}. 
    \item This is an important point that we should have discussed more. Our analysis in \rev{Figure \ref{fig:vary_space_performance} and Figure \ref{fig:vary_space_efficiency}} of our revised paper, shows that AutoFJ is about 40\% slower than Excel with  24 discrete configurations. Because Excel is considered as ``real-time'', our latency should still be reasonable (and with scope for further optimization using more careful engineering, for example). This is in contrast to other state-of-the-art approaches from the literature like ZeroER, Magellan and FW, which are up to 3x slower than AutoFJ and Excel. At the cost of a small increase in latency, AutoFJ is noticeably better in terms of quality (e.g., 0.700 vs. 0.659 in Precision-Recall-AUC, which is statistical significant with p=0.001, and 0.582 vs. 0.546 in recall, with p=0.08). All these additional numbers are detailed in the full paper we shared along with our code for reproducibility\footnote{https://www.dropbox.com/sh/myiees5wv716n2f/AAA-Px5AVDxt4kXJoKXnskSxa?dl=0}. 
    When using a full space of all 140 possible configurations, AutoFJ PR-AUC goes up to 0.715 (from 0.700) and recall goes up to 0.624 (from 0.582), at the cost of a 2-3x increase of latency. These are interesting trade-offs between quality and latency, and we now report details of these experiments in \rev{Section \ref{sec:single_column_evaluation_results}}.  
\end{itemize}


\bigskip
\begin{tcolorbox}
\textbf{O3: It would be very interesting to see whether your estimated and actual precision/recall values match. Consider adding a study that shows the development of the estimated vs actual values over time (algorithm iterations?) or as an additional field in Table \ref{table:single_performance}.}
\end{tcolorbox}

\stitle{Response.} This is a good suggestion. We added this evaluation of estimated and actual precision/recall as suggested, and results show that the two indeed indeed match very well. Specifically, in the revision, we computed the Pearson correlation coefficient between the actual precision and the estimated precision over all iterations in the AutoFJ algorithm for each dataset.  The average Pearson correlation of precision turns out to be very high at 0.894, which indicates that the actual/estimated precision indeed match very well across iterations. (Detailed results are added as \rev{as an additional column called PEP-CC in Table \ref{table:single_performance}}).

We also compute the correlation coefficient between the actual/estimated recall over iterations, which is also very high at $0.938$, again suggesting that our estimation is indeed accurate across all dataset and algorithms iterations (Detailed results shown in the \rev{RER-CC column in Table \ref{table:single_performance}}).

\bigskip
\begin{tcolorbox}
\textbf{O4: One of the core problems in ER are missing attribute values. How does your technique handle that in multi-column joins?}
\end{tcolorbox}

\stitle{Response.} 

\begin{itemize}
    \item In our experiments,  when computing distances for two strings where one is a missing value, we take the conservative approach of assigning max distances, which is an approach also used in the literature (e.g.\cite{dong2005reference, talburt2011entity}). We have added this detail to the experimental setup \rev{in Section \ref{sec:multicol_setup}}.
    \item Crucially, our multi-column AutoFJ algorithm (in Algorithm \ref{alg:autofj_multi_column}) can automatically determine that columns with many missing values are less useful, because joins on such columns tend to produce high distance values and leading to less number of record-pairs to be joined (low estimated recall), making our algorithm to automatically assign lower importance-weights to such columns. We have added this discussion to \rev{ Section~\ref{sec:multi-column-algorithm}}. 
    \item This expected behaviour is further validated empirically in our experiments -- columns with missing values are usually either left unused or assigned lower weights by our algorithm (please see \rev{the discussion of the effectiveness of column selection in \rev{Section \ref{sec:multicol_results}}}).
\end{itemize}



\bigskip
\begin{tcolorbox}
\textbf{
A1: Multi-column experiments
In Sec. \ref{sec:multicol_results} the authors state that AutoFJ "remains the best method". However, looking at the per-dataset results, one can observe that active learning is the best choice in 6/8 cases, AutoFJ is the best choice on average. Please consider adjusting your observations to reflect this more accurately.}
\end{tcolorbox}

\stitle{Response.} This is a good catch and we have updated our description in \rev{Section \ref{sec:multicol_results}} to make it more precise. 
%In particular, we have now stated that, on average, \textsc{AutoFJ} significantly outperforms other unsupervised methods and achieves comparable performance as supervised methods. 

\bigskip
\begin{tcolorbox}
\textbf{A2: Write-up
There are several opportunities in the current version to improve the flow and at the same time to make space for the additional experiments and explanations requested above. Here are a few suggestions: (1) Figure 1 is not necessary to understand the problem statement. (2) The introduction in general could be shortened, it's nearly 3 pages long. For example, paragraph Auto FuzzyJoin is mostly covered in the problem statement in Sec 2. Consider merging it with the previous paragraph. (3) Paragraph ``Highlights of our approach'' in the introduction is more suitable as part of the preliminaries than the introduction as it describes desiderata of the solution. (4) Sec 4: Why do you introduce a new example, can you utilize or replace any of the examples in Figure 3 instead? (5) The algorithm description in 4.2 could be shortened, there is  a figure, a textual description and an example. Consider dropping one of those.}
\end{tcolorbox}

\stitle{Response.} We have made these changes as suggested.  

\begin{itemize}
    \item We have \rev{removed the original Figure 1} to make space for additional materials.
    \item We have \rev{merged the  original ``Auto-FuzzyJoin'' paragraph in introduction} with the previous paragraph, as suggested. 
    \item We have \rev{``removed the Highlights of our approach''}.
    \item Regarding why a new example in Section 4 is introduced, unfortunately we could not re-use previous examples because all previous examples are single-column cases while Section 4 requires an example for multi-column joins. 
    \item We have cut the textual description of the algorithm \rev{in Section 4.2}. 
\end{itemize}

\bigskip
\begin{tcolorbox}
\textbf{A3: Nits: (1) Sec 1, sentence before 'Key Insights' -> Brackets are superfluous. (2) Sec \ref{sec:alg_compared} Magellan[29]: ... [29]. -> Double reference in one sentence.}
\end{tcolorbox}

\stitle{Response.}  We have addressed these issues.

\bigskip
{\huge \stitle{Response to Comments by Reviewer 2}}

Since there are substantial content in this section, we will first discuss the comments listed as ``critical''  (O1, O6, O7, O10) by the reviewer (in Q8 of the review), before describing our response to all other comments. 

\bigskip
\begin{tcolorbox}


\textbf{O1: The key insight ``Leverage Reference-Tables" relies on an assumption that all the elements in L should not be similar, which is not mentioned in the paper. With this assumption, the approach proposed in this paper can only work for a very limited cases. For the key insight "Leverage Reference-Tables", authors only mention one requirement that elements in L should have few or no duplicates. However, it is not enough. Recall the example, if l1 and l5 are similar but not the same, then both l1 and l5 can coexist in L, then this key insight breaks. Am I missing anything?}
\end{tcolorbox}

\stitle{Response.}

\begin{itemize}
    \item We have clarified this aspect in  \rev{the ``Leverage Reference-Tables'' paragraph in Section 1} of the revision, and we will explain this in a bit more detail below to clarify the confusion (likely caused by the way our example was originally written in that paragraph).
    
    
    \item Our key insight/assumption is that the reference-table L should typically have few or no duplicates, but importantly, records in L *can* be similar (the presence of similar records in fact works to our advantage). To see why this is the case, we revisit the example in Figure 2(b) that was mentioned in reviewer's comment above. We copy Figure 2(b) below, for ease of reference.
    
\begin{figure}[h]
    \centering
    {\includegraphics[width=0.6\columnwidth]{images/ex-2.png}}
    \vspace{-2mm}
    \caption*{The original Figure 2(b) taken from our paper.}
\end{figure}
    
    \indent In this example, table L on the left has many highly similar records (e.g., $l_1$: ``Super Bowl XX Championship Game'' and $l_2$: ``Super Bowl XXI Championship Game'' that diff by only one letter, etc.). The presence of such similar records is totally fine and works to our advantage, because these highly similar L records essentially ``teaches'' our algorithm, that ``Edit-distance <= 1'' is not a good join condition here, because if it were a good join condition, we could apply it to pairs-of-records in the reference-table L, and would be seeing a lot of ``self-joins'' in the table L (e.g., $l_1$ fuzzy-joins with $l_2$ and $l_3$, etc.). A large number of such self-fuzzy-joins would  imply that these reference-records correspond to identical real-world entities (duplicates), and thus violating our key assumption that table L has few or no duplicates, making us to conclude that ``Edit-distance <= 1'' is not a good fuzzy-join condition on this particular dataset (even though in most other scenarios it is generally safe to perform fuzzy-join with ``Edit-distance <= 1'').
    
    
    \indent Instead of using ``Edit-distance <= 1'', our algorithm would search for alternative distance functions, and would find Jaccard-containment (with word-tokenization) to be a good distance-function for fuzzy-join on this dataset, because if we set ``Jaccard-containment == 1'' as the requirement, we would not be able to ``self-fuzzy-join'' any record-pairs in L (indicating that this fuzzy-join is likely ``safe'' following the same analysis above), and at the same time this allows us to join $(l_5, r_5)$ and $(l_6, r_6)$ correctly, which are indeed correct records to join, without producing false-positive joins on this difficult dataset.
    
    We highlight that in this process above, AutoFJ dynamically infers good/bad join configurations (e.g., what distance-functions to use), which is significantly different from other algorithms (e.g., Excel) that typically employ static distance-functions that would produce many false-positives here (such as joining $l_1$ and $r_1$).
    
    And as can be seen from the analysis above, having high-similar records in L (that actually corresponds to different real-world entities) is not a requirement for our algorithm to work, and in fact the presence of such similar records works in the favor of our AutoFJ algorithm, because it can leverage such information to reliably determine that certain fuzzy-join configurations would likely be ``bad'' (with too many false-positives through self-fuzzy-joins).
    
    \item Finally, we would like to stress our work is built on only one requirement that the reference-table L has few or no duplicates. This is something we observe to be true in most real data sets -- for example, in the well-known public repository of ER data sets compiled by Prof. AnHai Doan's group (https://sites.google.com/site/anhaidgroup/useful-stuff/data), we find this reference-table assumption holds on 26 out of 29 datasets listed on the web-page, making our approach to be applicable on 26/29 of these test cases. We have added this as a new discussion in \rev{Section~\ref{sec:many-to-one-join}}.
\end{itemize}



\bigskip
\begin{tcolorbox}
\textbf{O6: All the 50 datasets are generated from one single souce DBPedia, which seems all the datasets have similar distribution and property. It is highly suggested to include more different datasets. E.g., DBLP and Fodors-Zagat datasets utilized in ZeroER.}
\end{tcolorbox}

\stitle{Response.} In the original paper we submit, in addition to the 50 new datasets from DBPedia,
we also compared extensively using popular datasets from the literature, including DBLP and Fodar-Zagat mentioned in this comment, as well as many others (Abt-Buy, RottenTomato-IMDB, BeerAdvo-RateBeer, Amazon-BarnesNobel, iTunes-Amazon, BabiesRUs-BuyBuyBaby, etc.). Detailed comparisons on these data sets can be found in Table 3 and 4, and we request the reviewer to kindly review our experimental results there.



\bigskip
\begin{tcolorbox}
\textbf{O7: Missing many well-known competitors in experiments. E.g., ECM and PPjoin. They are all unsupervised methods. Please add them.}
\end{tcolorbox}
\stitle{Response.} We have added ECM and PPjoin as two additional baselines as suggested, for both single-column fuzzy join and multi-column fuzzy join settings. Experimental results for the two approaches can be found in \rev{Table \ref{table:single_performance}} and \rev{Table \ref{table:multi-column}}. Our results show that these two methods are substantially inferior in terms of fuzzy-join quality,
because ECM binarizes features, which loses information, while PPJoin is an efficient algorithm for Jaccard-similarity join, which is not as flexible and does not perform well on scenarios where other distance functions are needed (e.g., Edit-distance for typos, Jaccard-contaiment for subset-superset, etc.). The efficiency results of both methods are included in \rev{Figure \ref{fig:efficiency}}.




\bigskip
\begin{tcolorbox}
\textbf{O10: In "Varying Target Precision" and "Efficiency Analysis" it makes no sense to only compare with Excel. Especially for the Efficiency experiments.}
\end{tcolorbox}

\stitle{Response.} We have added the suggested comparisons with all other baselines in \rev{Figure \ref{fig:vary_target}}, so that readers can have a complete picture of the results (we originally showed results comparing with Excel only, because Excel is the only method that comes close in terms of join quality).  \rev{Figure \ref{fig:vary_target}} shows that as we vary the target precision, our approach remains the best (by a substantial margin) compared to all other methods. The running time of AutoFJ is competitive, and remains faster than other state-of-the-art methods from the literature, such as ZeroER (unsupervised) and Magellan (supervised). 



\bigskip
\begin{tcolorbox}
\textbf{O2: The conclusion that "whether we can perform unsupervised fuzzy-joins without additional constraints like reference tables, we show a negative result that this is in general impossible" is not very clear. What do you mean by constraints like reference tables? Please carefully quantify them.}
\end{tcolorbox}
\stitle{Response.}
We have rephrased this part  \rev{in Section~\ref{sec:problem}} to make it more clear. Intuitively, because of the presence of a reference-table L that should have few duplicates, we know the fuzzy-join configurations we select should not produce too many self-fuzzy-joins for record-pairs in L, as these would imply duplicates in L (explained in detail in our response to O1 above). This intuition would serve as a powerful ``constraint'', to prevent our algorithm from using fuzzy-join configurations that are too ``loose'' (or join more than what is correct). (We have an additional result to show that some forms of ``constraints'' would be necessary for unsupervised fuzzy-joins/entity-resolution, which is perhaps out of scope and is described in our full version\footnote{https://www.dropbox.com/sh/myiees5wv716n2f/AAA-Px5AVDxt4kXJoKXnskSxa?dl=0} submitted together with our code for reproducibility).

\bigskip
\begin{tcolorbox}
\textbf{O3: Proof of Theorem \ref{theorem:rmfj} (was Theorem 2.6 in our original paper) should be added to make the paper self-contained.}
\end{tcolorbox}

\stitle{Response.} We have added the proof of the theorem to the paper in \rev{Section \ref{sec:problem_definition}} as suggested.

\bigskip
\begin{tcolorbox}
\textbf{O4: The "complete"/"incomplete" of L is quite confusing. Given an L, it should always be complete afaik. Actually what is the definition of "complete", it seems you never define it.}
\end{tcolorbox}

\stitle{Response.} This is a good clarification that we have now made in the paper. Intuitively, a left table L is considered ``complete'' if every record in $R$ has a corresponding record to join in $L$, and conversely L is ``incomplete'' if some records in $R$ cannot join with any record in $L$. We emphasize that our approach does not rely on $L$ being complete, and it works equally well when $L$ is incomplete as we have shown in our experiments in Figure 5(c). We introduce this intuitive notion of complete/incomplete $L$ only to better explain our techniques (as we start our discussion with the simpler scenario of a complete $L$). We have made these clarifications in the revised paper.

%\textcolor{purple}{We have clarified the definition of ``complete" in the paper. A reference table (L) is considered to be complete if for every record in table R, we can find its matched record in L.}

\bigskip
\begin{tcolorbox}
\textbf{O5: In Figure \ref{fig:double_distance} (was Figure 4 in our original paper), "The more records in the 2d-ball, the more unreliable the join is", why? what is the intuition behind it? More records in the 2d-ball only mean it has more matchings.}
\end{tcolorbox}

\stitle{Response.} Indeed that more records in the 2d-ball means more matches, but importantly these matches are between pairs of $L$ records, and like we illustrated in our response to $O1$ above, fuzzy-matches between $L$ and $L$ records indicate that either (1) these matches are true matches, which would essentially make them duplicate records in $L$, violating a key property of the reference-table $L$ that it should have few or no duplicates, and thus should not happen, or (2) our fuzzy-matching criteria is too ``loose'' that produces false-positives between $L$ and $L$ records.

Because (1) should not happen given reference table $L$, we know (2) must have happened and our fuzzy-join conditions are too ``loose'', if we see more records in the 2d-ball, making us to conclude that such joins prone to false-positives and the results are unreliable.

We have clarified this intuition in \rev{Section~\ref{sec:estimate_precision_recall}}. Additional explanations (e.g., why triangle-inequality leads us to use 2d-balls are needed as opposed to 1d) can also be found in the section.

% show that 

\bigskip
\begin{tcolorbox}
\textbf{O8: For AR, how to break tie? It is not mentioned in the paper. If there are more than one pairs with the same prediction, how to choose the recall? It will significantly change the results.}
\end{tcolorbox}

\stitle{Response.} We have added these new details below to the paper in \rev{Section \ref{sec:evaluate_metrics}}. 

\begin{itemize}
\item We have been extremely careful in ensuring that Adjusted recall (AR) is computed in a way that is always favorable to baseline methods.  Specifically, when computing AR, if a baseline has ties in precision (i.e., two score-thresholds producing the same precision but different recall), we always report the highest possible recall among all such ties as the AR number for this baseline, which clearly favors baselines (our approach reports a true-recall when it stops iterating, which does not require adjustments).

\item In addition, there may be cases where our AutoFJ produces a recall R=0.8 at precision P=0.9, while a baseline B may not have an identical result to match in terms of precision -- e.g., the baseline B may have (R=0.75, P=0.89) and (R=0.7, P=0.91), neither of which matches perfectly with AutoFJ's P=0.9. In such cases, we look for closest precision value that is below 0.9 to ensure that the AR is more favorable to baselines. In this particular example, we would report AR=0.75 for B, even though its precision level 0.89 is lower than AutoFJ's 0.9.

%both over 0.9 and below 0.9, and pick the one with the highest recall as the AR number for baseline B. In this particular example, we would report AR=0.75 for B, even though its precision level 0.89 is lower than AutoFJ's 0.9.

\item Finally, to avoid any doubt on the (favorable) adjustments we make in AR for baselines, we have added comparisons using Precision-Recall-AUC, between AutoFJ and baseline methods. Our observed quality improvement in AR is consistently observed in this AUC evaluation -- AutoFJ AUC is 0.715, compared to the next-best unsupervised method (Excel) at 0.658, and the best supervised method (Magellan) at 0.659.  (Detailed numbers and case-by-case breakdown are shown in Table 5 of our full version\footnote{https://www.dropbox.com/sh/myiees5wv716n2f/AAA-Px5AVDxt4kXJoKXnskSxa?dl=0}). We believe this should indeed validate our observation that AutoFJ indeed produces higher-quality join results (in AR or AUC) compared to alternative methods.
\end{itemize}


\bigskip
\begin{tcolorbox}
\textbf{O9: In Robustness Test (3): L Incompleteness. If the records in L are randomly removed, how can AutoFJ keeps the same recall while decreasing precisions? }
\end{tcolorbox}
\stitle{Response.} This is a good question that we should clarify -- our recall is defined in relative terms (relative to all  ground-truth join pairs between $L$ and $R$, what fraction are being joined correctly). As a result, irrespective of how many  records we remove from $L$, the best possible recall is always 1.0. We have clarified this \rev{in Section~\ref{sec:single_column_evaluation_results}} now. 



\bigskip
{\huge \stitle{Response to Comments by Reviewer 3}}

\bigskip
\begin{tcolorbox}
\textbf{O1: At the core of the presented solution and the experimental analysis lies a user-determined performance target with respect to precision. The goal is to maximize recall for the desired level of precision. This choice is not justified and seems counter-intuitive. It would make more sense to predetermine the desired level of recall (i.e., "find 90\% of all matches") and to maximize precision accordingly.}
\end{tcolorbox}


\stitle{Response.} Indeed this alternative formulation of targeting a desired recall level would also be highly useful and is a dual version of our problem. There are minor technical difficulties in the alternative version however (such as it is more difficult to accurately estimate relative-recall compared to precision used in our version), which is perhaps also why the version of problem we study (targeting precision) is more commonly-used in the ER literature (e.g.~\cite{DBLP:dblp_conf/sigmod/ArasuGK10,bellare2012active} also targets a given precision level while maximizing recall). 

We should highlight that in addition to research papers, popular software packages like Magellan (Section 3.1 of Magellan~\cite{konda2016magellan}) also considers targeting a given precision-level as an explicit scenario. 

We fully agree with the reviewer that the alternative version is highly useful and deserves future attention from the research community. We have added a discussion of this \rev{at the end of Section~\ref{sec:problem_definition}}.

\bigskip
\begin{tcolorbox}
\textbf{O2: Certain critical aspects of the presented solution are not discussed in detail. First of all, how are the results of different joins/matching rules merged? If l\_1 matches (i.e., has the minimum distance) with r\_1 for a configuration using Jaccard distance and with r\_2 for a configuration using edit distance, which pair will be selected when merging the results of these two configurations? Also, what is the space and time complexity of Algorithms 1 and 3 (was Algorithm 2 in our original paper) with respect to the input size (i.e., number of records in L and R)? Finally, what is the exact algorithm that is used for learning negative rules? Does it compare all pairs of records in the reference table? When is it called in Algorithm 1 and 3? How is it configured? E.g., does it use lowercase and stemming for preprocessing? Does it use 2-gram, 3-gram or Space tokenization?}
\end{tcolorbox}
\stitle{Response.} There are multiple questions in O2 worth clarifying, and we will address them separately below.

\begin{itemize}
    \item Regarding conflict resolution, to make things clear, we distinguish between two scenarios below. 
    \begin{itemize}
        \item  The first scenario is when one record in $L$ ($l_1$) joins with multiple records in $R$ ($r_1$ and $r_2$) using different configurations. This scenario is fine and would not be considered as a conflict (e.g., $l_1$ could be ``David M. Smith'' that fuzzy-joins with $r_1$ ``Mr. David M. Smith'' using Jaccard, and at the same time also fuzzy-joins with $r_2$ ``Dave M. Smith'' using Edit). This scenario is perfectly consistent with the many-to-one fuzzy join semantics  defined in Definition~\ref{def:many-to-one-join}. 
    
    \item The second scenario is when a record in $R$ (written as $r_1$) joins with multiple records in $L$ ($l_1$ and $l_2$) under different configurations. This scenario should not happen because our reference table $L$ should have few or no duplicates, and having $r_1$ join with both $l_1$ and $l_2$ would imply that $l_1$ and $l_2$ should also join (by transitivity) and making them duplicates in $L$, thus violating the property above. (This was explained in our Definition~\ref{def:many-to-one-join}). When such conflicts do occur from multiple configurations, we  resolve them as follows. Consider a record $r_1 \in R$ that joins with $l_1$ under $C_i$, and joins with $l_2$ under $C_j$, with $l_1 \neq l_2$. We use our precision estimate in Equation~\eqref{eqn:r_prec_C} to compare $precision(r_1, C_i)$ and $precision(r_1, C_j)$, and pick the more confident one as the join result. This approach is now \rev{highlighted at the end of Section~\ref{sec:estimate_precision_recall}} when we discuss precision/recall estimation for a set of configurations.
    \end{itemize}
   

    
 
    \item Regarding space and time complexity of Algorithm \ref{alg:autofj_single_column} and Algorithm \ref{alg:autofj_multi_column} (was Algorithm 2 in our original paper), we now have added the time and space complexity for Algorithm \ref{alg:autofj_single_column} and Algorithm \ref{alg:autofj_multi_column} \rev{at the end of Section \ref{sec:auto_fj_algorithm_single_column} and Section \ref{sec:multi-column-algorithm}}, respectively. 
    %%
    We use $|S|$ to denote the number of discrete configurations ($|S| = 140$ in our experiments), $|L|$ to denote the size of the left reference table, $|R|$ to denote the size of the right table, $m$ to denote the number of columns in the multi-column setting, and $g$ to denote the step size for the column weight search ($g = 10$ in our experiments). The time (and space) complexity of Algorithm 1 is $O(|S||L|\sqrt{|L|} + |S||R|\sqrt{|L|})$. The time complexity of Algorithm 3 is $O(m^2g(|S||L|\sqrt{|L|} + |S||R|\sqrt{|L|}))$, and its space complexity is $O(m(|S||L|\sqrt{|L|} + |S||R|\sqrt{|L|}))$ (the extra factor of $m$ is because we need to pre-compute distances for all $m$ columns).
    
    
    \item Regarding the exact procedure of negative rule learning and where it is applied, we have made the following improvements. 
    
    \begin{itemize}
            \item     The negative rules are learned and applied after the blocking step in Algorithm~\ref{alg:autofj_single_column} for single-column joins, and Algorithm~\ref{alg:autofj_multi_column} calls  Algorithm~\ref{alg:autofj_single_column} as a sub-procedure. We have \rev{updated the pseudo-code of  Algorithm~\ref{alg:autofj_single_column}} to reflect this. For details regarding blocking, please see our response to R3.O3 below that specifically explains the blocking step.
            
            
        \item We have now added a new \rev{Algorithm~\ref{alg:negative_rules} that shows the pseudo-code for learning negative rules}, which takes as input LL (the left-left record pairs after blocking) and LR (the left-right record pairs after blocking).   It first preprocesses the input records by using lowercasing, removing punctuation, and applying stemming. It will then learn negative rules based on the input LL (where records are tokenized using space). Finally, the learned negative rules are applied to the fuzzy-joined LR (where records are tokenized using space), to prune away pairs that violate the learned negative rules.
        %We have added these details and summarized the algorithm for learning and applying negative rules in .


    \end{itemize}
    
\end{itemize}





\bigskip
\begin{tcolorbox}
\textbf{O3: The proposed solution lacks a way of pruning large parts of the search space of parameter configurations, even though its size is exponential in the number of parameters. For Algorithm \ref{alg:autofj_single_column}, there is a short discussion about efficiency optimizations at the end of Section 3.2, but more details are needed, as they merely seem to reduce the cost of a single parameter configuration, which is quadratic to the input size. More details are also needed for the configuration of the blocking method (e.g., lowercase, stemming, character or token n-grams) and for the experiments that led to this configuration. For Algorithm \ref{alg:autofj_multi_column} (was Algorithm 2 in our original paper), there is a significant pruning in the number of configurations that are considered, but still, the final computational cost seems very high.}
\end{tcolorbox}

\stitle{Response.} There are multiple questions in O3 that are all important. We will address them separately in the following, and have made improvements in our paper to clarify them.

\begin{itemize}
    \item Regarding the size of the configuration space (denoted as $|S|$ in our paper) and its impact on the performance of Algorithm 1 and 3:
    
    \begin{itemize}
        \item  Though the configuration space is in principle exponential in the \textit{types} of parameters, in practice there is only a total of 4 types of parameters (pre-processing, tokenization, token weighting, and distance function), so the parameter space is really exponential in a very small constant (4). Furthermore for each type of parameter there is only a small number of choices (e.g., there are not that many tokenization-methods, or distance-functions, etc.). We have surveyed the literature extensively, to enumerate common choices of these parameters, which are summarized in Table 1 and Figure 1 of our paper. Note that we have the very intention to be exhaustive, and have included choices such as word-embedding-based distances that are not very common for fuzzy-joins. In the end, even with an exhaustive search and a full cross-product of these 4 types of parameters, we get $|S| = 140$ total parameter-combinations, which is not a lot. (Note that some combinations are not permissible and have to be excluded, such as using word-tokenization with  character-based Edit-distance. A detailed explanation of how we arrive at the 140 number can be found in Section 5.1.3 of our paper).   We have added a discussion on this in our revised \rev{Section~\ref{sec:alg_compared}}.
        
        \item The time complexity of Algorithm 1 is $O(|S||L|\sqrt{|L|} + |S||R|\sqrt{|L|})$ and the time complexity of Algorithm 3 is $O(m^2g(|S||L|\sqrt{|L|} + |S||R|\sqrt{|L|}))$, which are now added \rev{at the end of Section \ref{sec:auto_fj_algorithm_single_column} and Section \ref{sec:multi-column-algorithm}}, respectively. As we can see, both algorithms have linear complexity with respect of $|S|$. 
        
    \item As suggested by the reviewer, pruning the search space of parameter-configurations are very useful directions of future work. For example, we could consider sampling L and R, and then estimate effectiveness of different parameters on the samples, to prune away ineffective parameters without needing to perform joins on full-tables. Similarly, we could resort to prioritized selection of parameters (e.g., via policies learned through reinforcement-learning) to prioritize our search in the promising subset of the parameter space. These are all very interesting directions for future work (our current system can handle the full 140 configurations reasonably well).
    \end{itemize}
    
   
    \item Regarding the details of blocking,  to design a strategy for blocking, we essentially need to determine a value for all four configuration parameters (preprocessing, tokenization, token weighting, and distance function) as well as the distance threshold used. We describe our choices used in blocking below, and details are added to the \rev{efficiency optimization paragraph in Section~\ref{sec:auto_fj_algorithm_single_column}}.

\begin{itemize}
    \item  For the preprocessing parameter, the tokenization parameter, and the weighting parameter, we use lowercase, 3-gram, and IDF, respectively. These parameter values are used because they are the most commonly used by our auto-tuned solutions. 
    %preprocessing, we use lowercase. For tokenization, we use 3-gram. For token weighting, we use  IDF. 
    
    \item  For deciding which similarity function to use for blocking, it  is a bit more involved since we need a similarity function that can be computed efficiently without actually enumerating all record pairs (or it would be quadratic and defeats the purpose of blocking). At the same time, we need a similarity function that can effectively identify tuple pairs that are unlikely to be matches.
    Our choice of similarity function is inspired by \textit{overlap blocker}, one of the blocking techniques used in Magellan \cite{konda2016magellan}. Overlap blocker uses the the number of tokens shared by two records as the similarity function, which can be computed efficiently using inverted index. Inspired by this method, we also use the shared tokens to compute the similarity, but instead of counting the number of tokens, we compute the sum of IDF weights of shared tokens. This avoids including tuple pairs that share many meaningless frequent tokens, such as ``the", ``an", which have lower IDF weights.
    
    
    \item Given our choice of similarity function above, we need to decide on a threshold value since it affects the number of candidate tuple pairs (e.g., a threshold value of 0 would return all pairs that share at least one common token, while a higher threshold value reduces the size of candidate tuple pairs at the risk of losing true positives). A good threshold value is likely dataset-dependent and cannot be a fixed threshold value. For this reason, we design an approach that avoids picking a specific threshold-value, but keeps the top-$\sqrt{|L|}$ matching $L$ records for each record in $R$ (which adapts to different datasets and determines thresholds dynamically). This choice of $\sqrt{|L|}$ makes sure that our blocking grows sub-linearly to input sizes, and at the same time keeps more candidates when we encounter a larger (and more difficult) $L$, which may have more number of confusing candidate records and thus the need to keep more candidates post-blocking. On this particular choice of  $\sqrt{|L|}$ (as opposed to other choices like $2\sqrt{|L|}$ or $3\sqrt{|L|}$), we have performed a sensitivity study in Figure~\ref{fig:block_sensitivity}, which shows that the performance of AutoFJ remains insensitive to different choices. 
    
    %Our intuition is that if a record in $R$ has corresponding record in $L$, then the corresponding record must be similar to  The similarity threshold affects the number of tuple pairs after blocking, but we would not expect users to tune the threshold. Therefore, instead of using a fixed similarity threshold, we sort the $L$ records by their similarity scores and only keep the top $\sqrt{|L|}$ records with the highest similarity scores.
    
    \item  We fully acknowledge that through this design process, we are not necessarily arriving at the best possible blocker. But at the same time, we do view blocking as an important but relatively orthogonal component -- alternative blocking methods can be plugged in and made to benefit our end-to-end system, and similarly the main technical contribution of our work (algorithms to auto-configure fuzzy-joins) can be plugged into other systems (e.g., Magellan) and produce benefits in a different context. Designing better blocking is a very important and orthogonal direction clearly worth more attention from the research community. We have added some of these discussions in our paper.  
\end{itemize}

\item Regarding the computation cost of Algorithm 3: Indeed, Algorithm 3 is slower than Algorithm 1 due to the need to consider multiple columns. %constant factor $O(m^2g)$ to tackle the multi-column join setting ($m$ is the number of columns and $g$ is step size for the column weight search). 
However, as discussed in Section 4, we have made substantial optimizations in Algorithm 3, resulting in significant improvements in efficiency over simple enumerations (reducing the complexity from exponential in column numbers to quadratic). We believe that the multi-column case presents an interesting spectrum of trade-offs between latency and quality -- e.g., using unit-column-weights would lead to fast join selection but inferior quality, while dynamic weights gives the best quality at the cost of increased run-time, and there are many other possible choices in between these two extremes. In this paper and for the multi-column join case, we focus on the most difficult and technically interesting variant of getting the best possible quality with dynamically-determined weights (simpler variants with unit-weights would be much more straightforward and omitted due to space). In the future, for given a latency requirement (e.g., 3 seconds), or a quality requirement, it would indeed be very interesting to look at the right strategy across this spectrum, which are promising directions for future work. 
    
    % In other words, it only keeps the tuple pairs that share at least $k$ tokens.
    
    % However,  this method has two weaknesses. First, the blocker may fail to filter some unmatches that share many frequent tokens, such as ``the", ``an". Second, it is hard to determine the parameter $k$. A larger $k$ would be more aggressive but may also lose many matches. We design our blocking technique with two improvement on the original overlap blocker to overcome these issues. First, instead of using the number of the share tokens, we add the IDF weight to each shared taken, and use the sum of the IDF weight as the similarity function. Since the frequent words have smaller IDF weight, even if two records share many frequent words, their similarity score would be small.
    % Second, instead of using a similarity threshold $k$, we sort the $L$ records by their similarity scores and only keep the top $\sqrt{|L|}$ records with the highest similarity scores. It is also interesting to investigate the automated blocking method without tuning parameters as a direction future research.  
    
    % \item \xu{Do we need to do or say anything about scalability in mult-colomn joins? }
\end{itemize}
% \textcolor{purple}{(1) 
% (2) We will provide more details on blocking. 
% (3) In the multi-col setting, the config space is indeed much larger, and is why our forward selection algorithm is important. We will give more details.}

\bigskip
\begin{tcolorbox}
\textbf{O4.1: Why is adjusted recall preferred over F-Measure? The former is suitable for the precision-target of auto-fuzzyjoin, but does not seem representative of the actual effectiveness of an ER solution. Assume that the desired level of precision is 0.90 and an ER method achieves 0.90 recall for 0.89 precision and 0.80 recall for 0.91 precision; adjusted recall considers only the latter performance, but the former one has significantly higher F-Measure (0.89 vs 0.85). I guess this is the reason why the performance of Magellan and DM over AB (the popular abt-buy benchmark dataset I guess) is much lower than that reported in the DeepMatcher paper, mentioning just one example. }
\end{tcolorbox}

\stitle{Response.} These are good points. To remove any doubt that AutoFJ's superior quality is due to the evaluation metrics (adjusted-recall), we have  (1) modified our procedure to compute adjusted-recall and made it even more favorable to baselines; and (2) added another metric, Precision-Recall-AUC, to compare different algorithms apple-to-apple. 

\begin{itemize}
    \item We have modified the procedure to compute adjusted-recall (AR) for baselines in \rev{Section \ref{sec:evaluate_metrics}}. For a given baseline, instead of using the precision value \textit{closest} to AutoFJ's precision (which could be both above or below AutoFJ's precision), we now use the closest precision value \textbf{lower than} AutoFJ's precision, and we report the corresponding recall as the adjusted recall for that baseline.  In the reviewer's example, the new AR computation procedure would choose  precision of 0.89 from another ER method to match AutoFJ's precision of 0.9, and then use that method's recall of 0.90 as its adjusted recall (which clearly favors all other methods we compare with).     We have updated the experiment results in \rev{Table \ref{table:single_performance}} and \rev{Table \ref{table:multi-column}}. It shows that our method can still significantly outperforms other methods based on the new AR (e.g., $0.624 - 0.562 = 0.062$ better than \textsc{Excel} and $0.624 - 0.495 = 0.129$ better than \textsc{AL} in Table \ref{table:single_performance}).
    
    %Then, if our recall is higher than the AR of baseline methods, it also indicates that we have a higher F-measure. However, if our recall is lower than the AR of baseline methods, it does not necessarily mean that our F-measure is lower, since our precision is higher. Hence, the new AR becomes more favorable for baselines than the standard F-measure. 

    
    \item We now report Precision-Recall-AUC scores as an additional evaluation metric (defined as the area under the Precision-Recall curves, which is a standard metric measuring result quality over the entire spectrum of precision/recall values).  A higher PR-AUC score generally correspond to higher recall/precision/ F-measure at different thresholds. The new metric is introduced in \rev{Section \ref{sec:evaluate_metrics}}. We also updated \rev{Table \ref{table:single_performance}} (last row) and \rev{Table \ref{table:multi-column}} (last row) to include results for PR-AUC (full details of these PR-AUC numbers across all datasets are included in the full version of our paper~\footnote{https://www.dropbox.com/sh/myiees5wv716n2f/AAA-Px5AVDxt4kXJoKXnskSxa?dl=0} that we submitted together with our code). For single column fuzzy joins, the results shows that our method remain the best based on the PR-AUC score ($0.715 - 0.658 = 0.057$ better than the best unsupervised approach \textsc{Excel}  and  $0.715 - 0.659 = 0.056$ better than the best supervised approach \textsc{Magellan}). For multi-column fuzzy joins, our method remain the best compared to other unsupervised method ($0.847-0.785 = 0.062$ better than \textsc{Excel}) and achieve comparable performance as supervised methods based on the PR-AUC score. 
    \item We hope these additional numbers and experiments provide more evidence that our approach indeed offers advantages in terms of join-quality, regardless whether the evaluation metric is AUC or precision-adjusted-recall. \item Finally to ensure reproducibility, we provide detailed instructions in our shared folder\footnote{https://www.dropbox.com/sh/myiees5wv716n2f/AAA-Px5AVDxt4kXJoKXnskSxa?dl=0} that allow reviewers to reproduce these numbers reported in the paper using the code we submitted for review.
\end{itemize}

\bigskip
\begin{tcolorbox}
\textbf{O4.2
Also, more emphasis should be placed on examining the time efficiency and the scalability of the proposed solution. At the moment, only Figure~\ref{fig:efficiency} presents the run-time of auto-fuzzyjoin, but this is not associated with the effectiveness performance in Table \ref{table:single_performance} or elsewhere. }
\end{tcolorbox}

\stitle{Response.} This is a good suggestion. We have made improvements in the revised paper by adding an evaluation on the efficiency of our algorithm in \rev{Section \ref{sec:single_column_evaluation_results}}, and associated the efficiency aspect with the effectiveness/quality of our algorithms. Specifically, we conducted an experiment where we vary the number of of configurations used by AutoFJ, from the full space with 140 configurations (shown in Table 1 and Figure 1), to a reduced subset with 24 configurations, to better understand the efficiency/effectiveness trade-off in our algorithms. As shown 
in \rev{Figure \ref{fig:vary_space_performance}}
and \rev{Figure \ref{fig:vary_space_efficiency}}, when we shrink the configuration space from 140 to 24 (the reduced configuration space is achieved by removing some options for the 4 parameters), our algorithm becomes 2x faster. The precision remain almost unchanged, while the recall and PR-AUC decrease slightly. We should highlight that even with the 24 core configurations, AutoFJ still substantially outperform the strongest baselines (e.g., Excel and Magellan), in terms of both AUC and adjusted-recall.

It is interesting to see that  the latency of our algorithm does not grow perfectly linearly with the number of configurations. This is because (1) different configurations may have different \textit{unit cost} in distance computation; and (2) for some distances, the computation can be shared with other distances, making the incremental cost of adding a distance sub-linear/sub-modular (e.g.,  jaccard, cosine, and dice distances all require the computation of token intersection, which is the most expensive part that can be shared between these distances). 

\bigskip
\begin{tcolorbox}
\textbf{O4.3: The datasets in Table \ref{table:single_performance} are generally small and given that they involve a single attribute, they are not typical of the data targeted by ER systems like Magellan, DM and AL.}
\end{tcolorbox}

\stitle{Response.} While our 50 new datasets from DBPedia are all single-columns (which we feel would still make an interesting benchmark set for the community), we also compared with 8 multi-column datasets (listed in Table~\ref{table:multicol_datasets}) used by previous ER systems, which showed that AutoFJ is competitive in terms of quality (by both AUC or adjusted-recall).

%We agree that practical ER tasks usually involve multiple attributes. We also conduct experiments on multi-column datasets (Table \ref{table:multicol_datasets}), which are typically used in by ER systems like Magellan, DM and AL.


\bigskip
\begin{tcolorbox}
\textbf{O4.4: 
In Ablation Study 1, it is mentioned that 0.587 is just 3.8\% lower than 0.625, which is not true. }
\end{tcolorbox}
\stitle{Response.} We should clarify that we used absolute difference ($0.625-0.587 = 0.038$). We have made sure that in the revised paper, our description is clear on whether a reported difference is in relative or absolute terms. (Note that due to changes of how we compute adjusted-recall in response to reviewer's O4.1 above, this number has been changed to 4.9 percentage-points accordingly). 

%We have now corrected it as percentage points.

\bigskip
\begin{tcolorbox}
\textbf{O4.5: 
Please also use statistical significance tests for comparing the performance of autofj with the baselines methods in Tables~\ref{table:single_performance} and~\ref{table:multi-column} (originally  Tables 2 and 3). }
\end{tcolorbox}
\stitle{Response.} We have performed upper-tailed paired t-tests for comparing AutoFJ with all alternative methods. Specifically, for each baseline method, we form a NULL hypothesis stating that the recall of AutoFJ is not better than that of an alternative method (with the alternative hypothesis being that the recall of AutoFJ is better). 

\begin{itemize}
    \item In single-column joins, we treat each dataset as an independent sample, and thus 50 datasets would generate 50 pairs of recall of AutoFJ and the AR of the baseline. This would allow us to compute a p-value for each baseline, where a small p-value indicating that we should reject the NULL hypothesis and lean towards believing that AutoFJ is indeed better than the baseline (A p-value smaller than 0.05 is generally considered as statistically significant). We show the p-value of this comparison for all baseline methods in the \rev{second to the last row of Table \ref{table:single_performance}}. As we can see, the p-values are all vanishingly small (the largest is 0.003), suggesting that AutoFJ is likely better than other methods in a statistically significant sense. 
    
    \item In multi-column joins, we again treat each dataset as an independent sample, and thus we have 8 pairs of recall of AutoFJ and the AR of the baseline. As we can see in \rev{the second to the last row of Table~\ref{table:multi-column}}, the p-values are all smaller than 0.05 except for AL (the active learning baseline). Indeed, AL has the closest average AR (0.844) compared to  the average recall of AutoFJ (0.858). However, we note that AutoFJ is a completely unsupervised approach while AL needs to actively engage users to label, and AL used 50\% of all ground-truth join pairs as labels in order to achieve the reported recall number (0.844), which is still no better than the unsupervised AutoFJ.
\end{itemize}




%We also perform upper-tailed T-Test over 50 datasets to verify the statistical significance of our results. The alternative hypothesis ($H_1$) assumes the mean of \textsc{AutoFJ}'s recall is greater than the mean of baseline's AR. As shown in the last row of Table \ref{table:single_performance}, the p-value of all baselines is smaller than 0.003, which shows the significance of our results.  



\bigskip
\begin{tcolorbox}
\textbf{O4.6:
Finally, it is not clear to me why the average precision fluctuates in  Figures~\ref{fig:robust_test1}, ~\ref{fig:robust_test3}, and~\ref{fig:block_sensitivity} (was Figures 6a, 6c and 6d in our original paper). Isn't target precision a predetermined measure?}
\end{tcolorbox}

\stitle{Response.} The target precision is indeed a predetermined measure for our algorithm. Figures~\ref{fig:robust_test1}, ~\ref{fig:robust_test3}, and~\ref{fig:block_sensitivity} performs what we call \textit{adversarial tests}, which artificially create extreme conditions (e.g., inserting a large amount of $R$ records totally irrelevant to the given $L$ and $R$) intended to test the robustness of our AutoFJ algorithm. These tests include inserting irrelevant records to $R$ (Figure~\ref{fig:robust_test1}), removing relevant records from $L$ (Figure~\ref{fig:robust_test3}), and  varying blocking factor (Figure~\ref{fig:block_sensitivity}, which is a sensitivity-test). These results show that under extreme adversarial situations, the actual precision obtained changes slightly from the normal settings (e.g., precision drop from 0.89 to 0.83), which however is not too significant and shows the robustness of our algorithms.

%In Figure~\ref{fig:vary_target}, we varied the target precision and compared different approaches. As we can see, the actual precision achieved by AutoFJ (the blue line with downward facing triangle) is very similar to the target precision as we vary the target. 

\bigskip
\begin{tcolorbox}
\textbf{A1: The term "fuzzy join" is a bit confusing, as it used to refer to Entity Resolution. A string or set similarity join is typically a well-defined problem on a single attribute (e.g., find all pairs with Jaccard similarity higher than 0.80), and the goal is to maximize its efficiency for the given similarity measure and threshold. Instead, the authors treat it as an open-ended problem defined over multiple attributes, which is better described by the term Entity Resolution.}
\end{tcolorbox}

\stitle{Response.}
%We agree that our fuzzy join problem is essentially the entity resolution problem with the additional constraint that $L$ table is a duplicate-free reference table. 
We agree that both fuzzy-joins are entity-resolution are used interchangeably in our setting, and depending on the specific context, entity-resolution may indeed be the better term. To us, fuzzy-join is the ``technical method'' with which we use to link-records together (e.g., Jaccard, Edit, etc., as pointed out by the reviewer), whereas ``entity-resolution'' can be used more broadly to refer to the general application of linking together related records, which can be agnostic to the underlying technical-method used (e.g., it could be deep-learning-based, graph-based, or fuzzy-join-based). As such, we have taken the suggestion and updated our terminology as appropriate in our paper (e.g., we state \rev{in Section~\ref{sec:many-to-one-join}} that our fuzzy join problem is really a technical method intended to be used in the application of entity resolution.


%We agree that fuzzy join is commonly used on joining based on a single attribute under a 

%The term ``fuzzy join'' and ``Entity Resolution'' are mostly interchangeable in the literature. We use ``fuzzy join'' in the paper because in our approach, we assume that the $L$ table is a reference table and the $R$ table is an input table. Our task is naturally to \textit{join} the $R$ table with the $L$ table. In contrast, the entity resolution is to identify the records corresponding to the same real-world entities from $L$ and $R$, where $L$ and $R$ are usually commutative.
\bigskip
\begin{tcolorbox}
\textbf{A2: The examples in Figure \ref{fig:ex} (was Figure 3 in our original paper) are a bit unclear and put more emphasis on recall than precision. The authors explain which pairs can be matched by which type of similarity join, but do not report the exact similarity thresholds. E.g., in Figure \ref{fig:ex-1}, $l_1$ is matched to $r_1$ with Jaccard distance, but the corresponding threshold is not mentioned. Most importantly, they do not discuss the precision of each join on the rest of the candidate matches. How many irrelevant pairs are matched when using the distance function and threshold as the one matching $l_1$ with $r_1$. This is rather important, especially when merging the results of multiple joins. By ignoring this aspect, these examples give the impression that we can/should come up with a different join/matching rule for every pair of matches.}
\end{tcolorbox}

\stitle{Response}. %Our approach indeed uses a union of join configurations, which can join different pairs with different join/matching rules. 
This is a good suggestion. We omitted detailed thresholds and the effect of applying these example join-rules in our original paper to make the example concise. For the pair $(l_1, r_1)$ and $(l_2, r_2)$ a Jaccard-distance $\leq$ 0.2 would match them together, which can be verified that would indeed not create any false-positive matches (assuming the learned negative-rules such as ``2007 $\neq$ 2008'' are applied as shown on the Figure). Similarly $(l_3, r_3)$ and $(l_4, r_4)$ would join with an Edit-distance $\leq 2$, which would again not create any false-positives (with the help of negative rules).  We have now clarified these details when we introduce the example in Figure \ref{fig:ex}, and highlight that this example does not imply that we would come up with a different joining rule for each matching pair. Rather, our algorithm will search for join configurations that individually can join as many pairs as possible (thus avoiding the situation of creating one join rule per match), while still retaining high precision. 

% different join/matching rule for different pair of matches. }
\bigskip
\begin{tcolorbox}
\textbf{A3: Some parts are repeated. E.g,. the example in Figure \ref{fig:ex-1} (was Figure 3a in our original paper), the baselines in 5.2.2. Please reduce the repetitive text to make room for more interesting content. Also, in Section 3.1, the paragraph "assuming a complete L" seems too long for its actual contribution. It could be shortened in few phrases. For the same reason, you could also shorten the lengthy introduction.}
\end{tcolorbox}

\stitle{Response}. We have removed the repeated parts and shorten the intro as suggested. 
\bigskip
\begin{tcolorbox}
\textbf{A4: There is a common numbering for Examples and Definitions in Section 2.}
\end{tcolorbox}

\stitle{Response.} Thank you for pointing this out, we have fixed this issue.
\bigskip
\begin{tcolorbox}
\textbf{A5: The paper needs a careful proof-reading, as there are several typos and missing or unnecessary words throughout the paper.}
\end{tcolorbox}

\stitle{Response.} We have carefully proofread the paper and fixed typos and missing/unnecessary words.
\bigskip
\begin{tcolorbox}
\textbf{A6: The authors should discuss the relation of their work with the publication "Auto-EM: End-to-end Fuzzy Entity-Matching using Pre-trained Deep Models and Transfer Learning"}
\end{tcolorbox}

\stitle{Response.} AutoEM~\cite{zhao2019auto} is a recent approach to EM using transfer-learning. This approach first pre-train EM models for various attribute types from knowledge bases. For a newly given EM task, it then requires a small number of labeled training data for what is known as fine-tuning. AutoFJ is fully unsupervised in comparison. We have added this discussion in our related work in \rev{Section \ref{sec:related}}.

%which is the x-axis in Figure \ref{fig:vary_target}. The average precision in Figure \ref{fig:vary_target} is the actual precision that our algorithm achieves, which may be slightly different from the target. 
%Hence, it may fluctuate as we we vary the target precision.    


% \textbf{A2:  The examples in Figure 3 are a bit unclear and put more emphasis on recall than precision. The authors explain which pairs can be matched by which type of similarity join, but do not report the exact similarity thresholds. E.g., in Figure 3a, $l_1$ is matched to $r_1$ with Jaccard distance, but the corresponding threshold is not mentioned. Most importantly, they do not discuss the precision of each join on the rest of the candidate matches. How many irrelevant pairs are matched when using the distance function and threshold as the one matching $l_1$ with $r_1$. This is rather important, especially when merging the results of multiple joins. By ignoring this aspect, these examples give the impression that we can/should come up with a different join/matching rule for every pair of matches.}



% \end{document}


